Beyond Incompatibility: Trade-offs between Mutually Exclusive Fairness Criteria in Machine Learning and Law

Fair and trustworthy AI is becoming ever more important in both machine learning and legal domains. One important consequence is that decision makers must seek to guarantee a 'fair', i.e., non-discriminatory, algorithmic decision procedure. However, there are several competing notions of algorithmic fairness that have been shown to be mutually incompatible under realistic factual assumptions. This concerns, for example, the widely used fairness measures of 'calibration within groups' and 'balance for the positive/negative class'. In this paper, we present a novel algorithm (FAir Interpolation Method: FAIM) for continuously interpolating between these three fairness criteria. Thus, an initially unfair prediction can be remedied to, at least partially, meet a desired, weighted combination of the respective fairness conditions. We demonstrate the effectiveness of our algorithm when applied to synthetic data, the COMPAS data set, and a new, real-world data set from the e-commerce sector. Finally, we discuss to what extent FAIM can be harnessed to comply with conflicting legal obligations. The analysis suggests that it may operationalize duties in traditional legal fields, such as credit scoring and criminal justice proceedings, but also for the latest AI regulations put forth in the EU, like the Digital Markets Act and the recently enacted AI Act.

==> 04-plot-results-zalando.tex <==
\newcommand{\resultplotfactortwo}{.1}
\begin{figure}
	\centering
	\subfloat
	[Ideal ranking (a synthetic example).
	\label{fig:experiments:result:zalando:synthetic}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/synthetic_ranking.png}}
	\subfloat
	[Original ranking as shown on the Zalando website.
	\label{fig:experiments:result:zalando:real}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/real_ranking.png}}\hfill
	\subfloat
	[Ranking after applying \methodname $\theta^A=1$.
	\label{fig:experiments:result:zalando:condA}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/fairer_ranking100.png}}
	\subfloat
	[Ranking after applying \methodname $\theta^B=1$.
	\label{fig:experiments:result:zalando:condB}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/fairer_ranking010.png}}\hfill
	\subfloat
	[Ranking after applying \methodname $\theta^C=1$.
	\label{fig:experiments:result:zalando:condC}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/fairer_ranking001.png}}
	\subfloat
	[Ranking after applying \methodname $\theta^A = \theta^B = \theta^C$.
	\label{fig:experiments:result:zalando:compromise}]
	{\includegraphics[height=\resultplotfactortwo\textheight]{figs/zalando/fairer_ranking111.png}}
	\caption{ (Best seen in color).
		Product rankings with \texttt{low} and \texttt{high} visibility brands under different settings. 
		%
		Colors indicate group membership, stripes indicate a positive label, \ie these are the products customers find more relevant. 
		%
		Fig.~\ref{fig:experiments:result:zalando:synthetic} exemplifies an optimal outcome, where all relevant products are in the top positions, and the visibility of brands A and B is distributed according to their share of relevant products. 
		%
		Fig.~\ref{fig:experiments:result:zalando:real} shows the distribution of relevant (and non-relevant) products from \texttt{low} and \texttt{high} brands as shown by Zalando's ranking algorithm by the time of data collection.
		%
		We see that famous brands do indeed have an advantage over less-known brands, as there are almost no products from the \texttt{low} group in the first few bins.
		%
		Fig.~\ref{fig:experiments:result:zalando:condA}---\ref{fig:experiments:result:zalando:compromise} show how the ranking changes after \methodname is applied with different values for $\theta^A$, $\theta^B$, and $\theta^C$.
		%
		Depending on our preference for calibration, balance for the positive class, or balance for the negative class, we see varying degrees of visibility improvement for the \texttt{low} group.
	}
	\label{fig:experiments:results:zalando}
	\vspace{-3mm}
\end{figure}


==> 04-table-results-compas.tex <==
\begingroup
\begin{table}
	\small
\caption {\label{tab:experiments:results:result-table-compas} Results for the COMPAS experiments.}
\vspace{-4mm}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{7}{llccccc}}
\toprule
Data Set & Parameters & \multicolumn{3}{c}{Performance} & \multicolumn{2}{c}{Error Rates}   \\
\cline{3-5} \cline{6-7}
      &&  Accur. ($\Delta$)  & Precision ($\Delta$) &  Recall ($\Delta$)	& FPR ($\Delta$) & FNR ($\Delta$) \\
      \toprule
      COMPAS & $\theta^A = 1$ & 0.660 (\textcolor{forestgreen}{0.006}) & 0.658 (\textcolor{forestgreen}{0.004}) & 0.660 (\textcolor{forestgreen}{0.006}) & 0.273 (\textcolor{forestgreen}{-0.041}) & 0.424 (\textcolor{red}{0.038}) \\
        $\;\;\;$ male && 0.653 (0.000) & 0.653 (0.000) & 0.653 (0.000) & 0.315 (0.000) & 0.383 (0.000) \\
		$\;\;\;$ female && 0.689 (\textcolor{forestgreen}{0.032}) & 0.689 (\textcolor{red}{-0.006}) & 0.689 (\textcolor{forestgreen}{0.032}) & 0.131 (\textcolor{forestgreen}{-0.181}) & 0.658 (\textcolor{red}{0.255}) \\
		\midrule
		COMPAS & $\theta^B = 1$ & 0.660 (\textcolor{forestgreen}{0.006}) & 0.657 (\textcolor{forestgreen}{0.003}) & 0.660 (\textcolor{forestgreen}{0.006}) & 0.225 (\textcolor{forestgreen}{-0.089}) & 0.486 (\textcolor{red}{0.100}) \\
		$\;\;\;$ male && 0.654 (\textcolor{forestgreen}{0.001}) & 0.656 (\textcolor{forestgreen}{0.003}) & 0.654 (\textcolor{forestgreen}{0.001}) & 0.230 (\textcolor{forestgreen}{-0.085}) & 0.479 (\textcolor{red}{0.096}) \\
		$\;\;\;$ female && 0.682 (\textcolor{forestgreen}{0.025}) & 0.673 (\textcolor{red}{-0.002}) & 0.682 (\textcolor{forestgreen}{0.025}) & 0.209 (\textcolor{forestgreen}{-0.103}) & 0.528 (\textcolor{red}{0.125}) \\
		\midrule
		COMPAS & $\theta^C = 1$ & 0.660 (\textcolor{forestgreen}{0.006}) & 0.657 (\textcolor{forestgreen}{0.003}) & 0.660 (\textcolor{forestgreen}{0.006}) & 0.225 (\textcolor{forestgreen}{-0.089}) & 0.486 (\textcolor{red}{0.100}) \\
		$\;\;\;$ male && 0.654 (\textcolor{forestgreen}{0.001}) & 0.656 (\textcolor{forestgreen}{0.003}) & 0.654 (\textcolor{forestgreen}{0.001}) & 0.230 (\textcolor{forestgreen}{-0.085}) & 0.479 (\textcolor{red}{0.096}) \\
		$\;\;\;$ female && 0.682 (\textcolor{forestgreen}{0.025}) & 0.673 (\textcolor{red}{-0.002}) & 0.682 (\textcolor{forestgreen}{0.025}) & 0.209 (\textcolor{forestgreen}{-0.103}) & 0.528 (\textcolor{red}{0.125}) \\
		\midrule
		COMPAS & $\theta^A = \theta^B = \theta^C$ & 0.660 (\textcolor{forestgreen}{0.006}) & 0.657 (\textcolor{forestgreen}{0.003}) & 0.660 (\textcolor{forestgreen}{0.006}) & 0.225 (\textcolor{forestgreen}{-0.089}) & 0.486 (\textcolor{red}{0.100}) \\
		$\;\;\;$ male && 0.654 (\textcolor{forestgreen}{0.001}) & 0.656 (\textcolor{forestgreen}{0.003}) & 0.654 (\textcolor{forestgreen}{0.001}) & 0.230 (\textcolor{forestgreen}{-0.085}) & 0.479 (\textcolor{red}{0.096}) \\
		$\;\;\;$ female && 0.682 (\textcolor{forestgreen}{0.025}) & 0.673 (\textcolor{red}{-0.002}) & 0.682 (\textcolor{forestgreen}{0.025}) & 0.209 (\textcolor{forestgreen}{-0.103}) & 0.528 (\textcolor{red}{0.125}) \\
	  \specialrule{1.5pt}{1pt}{1pt}
      COMPAS & $\theta^A = 1$ & 0.656 (\textcolor{forestgreen}{0.002}) & 0.654 (0.000) & 0.656 (\textcolor{forestgreen}{0.002}) & 0.271 (\textcolor{forestgreen}{-0.043}) & 0.435 (\textcolor{red}{0.049})\\
      $\;\;\;$ Caucasian & & 0.670 (0.000) & 0.663 (0.000) & 0.670 (0.000) & 0.224 (0.000) & 0.501 (0.000) \\
      $\;\;\;$ Afr.-Amer. & & 0.642 (\textcolor{forestgreen}{0.004}) & 0.643 (\textcolor{forestgreen}{0.003}) & 0.642 (\textcolor{forestgreen}{0.004}) & 0.333 (\textcolor{forestgreen}{-0.107}) & 0.382 (\textcolor{red}{0.096}) \\
      $\;\;\;$ Hispanic & & 0.664 (0.000) & 0.650 (0.000) & 0.664 (0.000) & 0.201 (0.000) & 0.583 (0.000) \\
	  $\;\;\;$ Other & & 0.688 (\textcolor{forestgreen}{0.005}) & 0.684 (\textcolor{forestgreen}{0.019}) & 0.688 (\textcolor{forestgreen}{0.005}) & 0.224 (\textcolor{red}{0.076}) & 0.475 (\textcolor{forestgreen}{-0.156}) \\
      \midrule
      COMPAS & $\theta^B = 1$ & 0.656 (\textcolor{forestgreen}{0.002}) & 0.654 (0.000) & 0.656 (\textcolor{forestgreen}{0.002}) & 0.271 (\textcolor{forestgreen}{-0.043}) & 0.435 (\textcolor{red}{0.049})\\
		$\;\;\;$ Caucasian & & 0.670 (0.000) & 0.663 (0.000) & 0.670 (0.000) & 0.224 (0.000) & 0.501 (0.000) \\
		$\;\;\;$ Afr.-Amer. & & 0.642 (\textcolor{forestgreen}{0.004}) & 0.643 (\textcolor{forestgreen}{0.003}) & 0.642 (\textcolor{forestgreen}{0.004}) & 0.333 (\textcolor{forestgreen}{-0.107}) & 0.382 (\textcolor{red}{0.096}) \\
		$\;\;\;$ Hispanic & & 0.664 (0.000) & 0.650 (0.000) & 0.664 (0.000) & 0.201 (0.000) & 0.583 (0.000) \\
		$\;\;\;$ Other & & 0.688 (\textcolor{forestgreen}{0.005}) & 0.684 (\textcolor{forestgreen}{0.019}) & 0.688 (\textcolor{forestgreen}{0.005}) & 0.224 (\textcolor{red}{0.076}) & 0.475 (\textcolor{forestgreen}{-0.156}) \\
      \midrule
      COMPAS & $\theta^C = 1$ & 0.656 (\textcolor{forestgreen}{0.002}) & 0.654 (0.000) & 0.656 (\textcolor{forestgreen}{0.002}) & 0.266 (\textcolor{forestgreen}{-0.048}) & 0.443 (\textcolor{red}{0.057})\\
      $\;\;\;$ Caucasian & & 0.670 (0.000) & 0.663 (0.000) & 0.670 (0.000) & 0.224 (0.000) & 0.501 (0.000) \\
      $\;\;\;$ Afr.-Amer. & & 0.642 (\textcolor{forestgreen}{0.004}) & 0.643 (\textcolor{forestgreen}{0.003}) & 0.642 (\textcolor{forestgreen}{0.004}) & 0.333 (\textcolor{forestgreen}{-0.107}) & 0.382 (\textcolor{red}{0.096}) \\
      $\;\;\;$ Hispanic & & 0.664 (0.000) & 0.650 (0.000) & 0.664 (0.000) & 0.201 (0.000) & 0.583 (0.000) \\
      $\;\;\;$ Other & & 0.683 (0.000) & 0.665 (0.000) & 0.683 (0.000) & 0.148 (0.000) & 0.631 (0.000) \\
      \midrule
      COMPAS & $\theta^A = \theta^B = \theta^C$ & 0.656 (\textcolor{forestgreen}{0.002}) & 0.654 (0.000) & 0.656 (\textcolor{forestgreen}{0.002}) & 0.271 (\textcolor{forestgreen}{-0.043}) & 0.435 (\textcolor{red}{0.049})\\
      $\;\;\;$ Caucasian & & 0.670 (0.000) & 0.663 (0.000) & 0.670 (0.000) & 0.224 (0.000) & 0.501 (0.000) \\
      $\;\;\;$ Afr.-Amer. & & 0.642 (\textcolor{forestgreen}{0.004}) & 0.643 (\textcolor{forestgreen}{0.003}) & 0.642 (\textcolor{forestgreen}{0.004}) & 0.333 (\textcolor{forestgreen}{-0.107}) & 0.382 (\textcolor{red}{0.096}) \\
      $\;\;\;$ Hispanic & & 0.664 (0.000) & 0.650 (0.000) & 0.664 (0.000) & 0.201 (0.000) & 0.583 (0.000) \\
      $\;\;\;$ Other & & 0.688 (\textcolor{forestgreen}{0.005}) & 0.684 (\textcolor{forestgreen}{0.019}) & 0.688 (\textcolor{forestgreen}{0.005}) & 0.224 (\textcolor{red}{0.076}) & 0.475 (\textcolor{forestgreen}{-0.156}) \\
      \specialrule{1.5pt}{1pt}{1pt}
      COMPAS & $\theta^A = 1$ &&&&& \\
      $\;\;\;$ $> 45$ & &&&&& \\
      $\;\;\;$ 25 -- 45 & &&&&& \\
      $\;\;\;$ $< 25$ & &&&&& \\
      \midrule
      COMPAS & $\theta^B = 1$ &&&&& \\
      $\;\;\;$ $> 45$ & &&&&& \\
		$\;\;\;$ 25 -- 45 & &&&&& \\
		$\;\;\;$ $< 25$ & &&&&& \\
      \midrule
      COMPAS & $\theta^C = 1$ &&&&& \\
      $\;\;\;$ $> 45$ & &&&&& \\
		$\;\;\;$ 25 -- 45 & &&&&& \\
		$\;\;\;$ $< 25$ & &&&&& \\
      \midrule
      COMPAS & $\theta^A = \theta^B = \theta^C$ &&&&& \\
      $\;\;\;$ $> 45$ & &&&&& \\
		$\;\;\;$ 25 -- 45 & &&&&& \\
		$\;\;\;$ $< 25$ & &&&&& \\
\bottomrule
\end{tabular*}
\end{table}
\endgroup


==> figs/compas/04-compas-transportmaps-gender.tex <==
\begin{figure}[t!]
	\centering
	\subfloat
	[Transport map to meet criterion A).
	\label{fig:experiments:result:compas:gender:condA}]
	{\includegraphics[height=\resultplotfactor\textheight]{figs/compas/gender/fairScoreReplacementStrategyCondA.png}}\hfill
	\subfloat
	[Transport map to meet criterion B).
	\label{fig:experiments:result:compas:gender:condB}]
	{\includegraphics[height=\resultplotfactor\textheight]{figs/compas/gender/fairScoreReplacementStrategyCondB.png}}\hfill
	\subfloat
	[Transport map to meet criterion C).
	\label{fig:experiments:result:compas:gender:condC}]
	{\includegraphics[height=\resultplotfactor\textheight]{figs/compas/gender/fairScoreReplacementStrategyCondC.png}}\hfill
	\subfloat
	[Transport map to meet fairness compromise with $\theta^A = \theta^B = \theta^C = 1/3$.
	\label{fig:experiments:result:compas:gender:compromise}]
	{\includegraphics[height=\resultplotfactor\textheight]{figs/compas/gender/fairScoreReplacementStrategyCompromise.png}}
	\vspace{-3mm}
	\caption{
		Also note, that raw scores have been normalized to $[0,1]$ during the procedure.
	}
	\label{fig:experiments:results:compas}
\end{figure}

